Differentiable Functional Program Interpreters

Programming by Example (PBE) is the task of inducing computer programs from input-output examples. It can be seen as a type of machine learning where the hypothesis space is the set of legal programs in some programming language. Recent work on differentiable interpreters relaxes the discrete space of programs into a continuous space so that search over programs can be performed using gradient-based optimization. While conceptually powerful, so far differentiable interpreter-based program synthesis has only been capable of solving very simple problems. In this work, we study modeling choices that arise when constructing a differentiable programming language and their impact on the success of synthesis. The main motivation for the modeling choices comes from functional programming: we study the effect of memory allocation schemes, immutable data, type systems, and built-in control-flow structures. Empirically we show that incorporating functional programming ideas into differentiable programming languages allows us to learn much more complex programs than is possible with existing differentiable languages.

==> background.tex <==
\section{Background}
\label{sect:background}

%% Do we need to say anything about TerpreT?
% We build on top of TerpreT~\citep{Gaunt16}, a recently introduced language to
% define program execution models.
% While this allowed us to easily experiment with many different program models,
% our conclusions are generally applicable.

The basic building block of functional programs is the function, and programs
are built by composing functions together.
In the following, we highlight some common features in functional programs
before discussing how to integrate them into an end-to-end differentiable model
in \rSC{sect:model}.

\paragraph{Memory Management}
Most modern programming languages eschew manual memory management and pointer
manipulation where possible.
Instead, creation of heap objects automatically generates an appropriate
pointer to fresh memory.
Similarly, built-in constructs allow access to fields of objects, instead of
requiring pointer arithmetic.
Both of these choices move program complexity into the fixed implementation of
a programming language, making it easier to write correct programs.

\paragraph{Immutable Data}
Functions are expected to behave like their mathematical counterparts, avoiding
mutable data and side effects.
This helps programmers reason about their code, as it eliminates the possibility
that a variable might be left uninitialized or accessed in an inconsistent state.
Moreover, no data is ever ``lost'' by being overwritten or mutated.

\paragraph{Types}
Expressive type systems are used to protect programmers from writing programs
that will fail.
Practically, a type checker is able to rule out many syntactically correct
programs that are certain to fail at runtime, and thus restricts the space of valid
programs.
Access to types helps programmers to reason about the behavior of their code.
In particular, the type system tells the programmer what kinds of data
they can expect each variable to contain.

\paragraph{Structured Control Flow}
A key difference between hardware-level assembly languages and higher-level
programming languages is that higher-level languages structure control flow using loops, conditional
statements, and procedures, as raw \texttt{goto}s are famously considered harmful~\citep{dijkstra1968}.
Functional languages go a step further and leverage higher-order functions to
abstract over common control flow patterns such as iteration over a recursive data
structure.
In an imperative language, 
% separating control flow from program logic is cumbersome, so
such specialized control flow is often repeated and mixed with other
code.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "nfp"
%%% End: 


==> straight_line_plot.tex <==
% This file was created by matplotlib2tikz v0.5.15.

